Closing the loop of SIEM analysis to Secure Critical Infrastructures

Critical Infrastructure Protection is one of the main challenges of last years. Security Information and Event Management (SIEM) systems are widely used for coping with this challenge. However, they currently present several limitations that have to be overcome. In this paper we propose an enhanced SIEM system in which we have introduced novel components to i) enable multiple layer data analysis; ii) resolve conflicts among security policies, and discover unauthorized data paths in such a way to be able to reconfigure network devices. Furthermore, the system is enriched by a Resilient Event Storage that ensures integrity and unforgeability of events stored.

==> architecture_old.tex <==
\section{Enhanced SIEM Architecture}\label{sec:architecture}
In this section we discuss the conceptual architecture of the enhanced version of the Security Information and Event Management (SIEM) system we propose in this paper. We present it through the block diagram in Fig. \ref{encSIEMArc}.
In Fig. \ref{encSIEMArc}, Hydroelectric Dam is the critical infrastructure we want to protect from cyber-attacks. These facilities host the information sources that we monitor through the SIEM. 
With GET we indicate the modules of the security collector software. The purpose of the GET is to generate security events by observing multiple layer data from the sources in the monitored infrastructure. The most relevant sources are physical sensors, logical access events, physical access events, network systems and logs from networked applications. The GET translates such events into a common format which is suitable for the central Correlator engine of the SIEM and for the Decision Support System. Also, the GET preprocess data in the collection points and detects anomalies in the cyber-physical systems (e.g. anomalies in the measured parameters). The Correlator analyzes the GET events in order to discover known attack sequences, i.e. sequences encoded through schematic rules and stored in the rule database of the SIEM. If one of the patterns of security breach is found, then the Correlator generates an alarm and sends it to the Decision Support System and to the Resilient Event Storage. Generated alarms contain information about the security breach, so they are useful for forensic purposes. In order to use the alarms generated and stored by the SIEM as evidence of cyber-crime, integrity and unforgeability must be guaranteed. The Resilient Event Storage is an intrusion and fault tolerant facility designed to ensure these two requirements; indeed, the RES is reliable in that it is able to keep record integrity, even if some components are compromised by an attack. 
The Decision Support System (based on XACML engine) ensures that the security policies established are not violated and it implements a resolution strategy when two policy are in conflict. Also, the Decision Support System uses a novel modeling approach based on the geometric representation of network device configurations (i.e. policies) which allows the computation of the reachability analysis using the concept of equivalent firewall. An equivalent firewall is a fictitious device, ideally connected directly to the communication endpoints, that summarizes the network connectivity between them. The reachability analysis is a approach useful to discover unauthorized data paths between hosts due to a misconfiguration of network infrastructure. Also, the reachability analysis is useful to compute new paths and insulate compromised links. The proposed model supports routing, filtering and address translation devices in a computationally effective way. If the Decision Support System discovers a misconfiguration, it activates the Reaction System that performs a control action on the scenario, e.g. a data path discovered and unauthorized is closed by inserting new firewalls rules.

\begin{figure}[htbp]
\centering
\includegraphics[scale=0.40]{figures/ConceptualArchitecture.png}
\caption{Enhanced SIEM Architecture}
\label{encSIEMArc}
\end{figure}
\input{correlatore.tex}

\input{DSSCNR.tex}

\input{DSSPOLITO.tex}

\input{Resilient.tex}

==> conclusionold.tex <==
\section{Conclusion and Future Work}
In this paper we discussed about the limitations of SIEM systems available today and we proposed a new enhanced SIEM architecture that overcomes the limitations identified. 
Also, in our study, we considered a misuse case that affects hydroelectric dam. As described in \cite{icscert1}, this critical infrastructure is highly exposed to cyber-attacks today. In future we will perform an extensive experimental campaign in order to validate the enhanced SIEM proposed using the scenario described.


==> rw.tex <==
\section{Related Work}\label{sec:rw}
SIEM \cite{general_siem} solutions are a combination of the formerly heterogeneous product categories of Security Information Management (SIM) and Security Event Management (SEM).
In particular, SEM systems are focused on the aggregation of data into a manageable amount of information with the help of which security incidents can be dealt with immediately, while SIM primarily focuses on the analysis of historical data in order to improve the long term effectiveness and efficiency of information security infrastructures \cite{william-SIEM}. 
 SIEM technology aggregates event data produced by security devices, network infrastructures, systems and applications. 
 %The primary data source is log data, but SIEM technology can also process other forms of data. Event data is combined with contextual information about users, assets, threats and vulnerabilities. The data is normalized, so that events and contextual information from heterogeneous sources can be correlated and analyzed for specific purposes, such as network security event monitoring, user activity monitoring and compliance reporting. The technology provides real-time security monitoring, historical analysis and other support for incident investigation and compliance reporting.
At the time of writing this paper, there are about 64 existing SIEM solutions \cite{siem-mosaic}, some of which are freeware whereas others are commercially available. Gartner Report \cite{gartner-siem} provides a overview about SIEM technologies widely adopted today and the report focuses on their strengths and weaknesses. The most widely used SIEM systems today are OSSIM and Prelude. OSSIM SIEM \cite{ossim-siem} is an Open Source SIEM which provides features as vulnerability and risk assessment, network and host intrusion detection, and file integrity monitoring. During 2012, AlienVault introduced Open Threat Exchange, which enables sharing of Internet Protocol (IP) and URL reputation information. A strong OSSIM limitation is about the correlation engine. In particular, the predefined correlation rules are focused primarily on Snort sensor data suite, so they cannot be used on other sensor suites. Also, the correlation rules are defined using XML syntax. This approach allows to write new correlation rules easily, but XML syntax limits the expressions that can be defined. Prelude SIEM \cite{prelude-siem} uses a correlation engine based on Python. The choice of a scripting language allows to overcome limitations of OSSIM due to XML syntax; however, Prelude does not perform risk assessment of events processed.



==> setupvalidation.tex <==
\section{System Setup and Validation}\label{sec:setval}
(All)
